OpenSalicon: An Open Source Implementation of the Salicon Saliency Model

In this technical report, we present our publicly downloadable implementation of the SALICON saliency model. At the time of this writing, SALICON is one of the top performing saliency models on the MIT 300 fixation prediction dataset which evaluates how well an algorithm is able to predict where humans would look in a given image. Recently, numerous models have achieved state-of-the-art performance on this benchmark, but none of the top 5 performing models (including SALICON) are available for download. To address this issue, we have created a publicly downloadable implementation of the SALICON model. It is our hope that our model will engender further research in visual attention modeling by providing a baseline for comparison of other algorithms and a platform for extending this implementation. The model we provide supports both training and testing, enabling researchers to quickly fine-tune the model on their own dataset. We also provide a pre-trained model and code for those users who only need to generate saliency maps for images without training their own model.

==> Makefile <==
## MAKEFILE FOR PHOTOGRAPHER PROJECT
## 7/15/2015

PDFLATEX	?= pdflatex -halt-on-error -file-line-error
BIBTEX		?= bibtex
MAKEGLOSSARIES ?= makeglossaries

ifneq ($(QUIET),)
PDFLATEX	+= -interaction=batchmode
ERRFILTER	:= > /dev/null || (egrep ':[[:digit:]]+:' *.log && false)
BIBTEX		+= -terse
else
PDFLATEX	+= -interaction=nonstopmode
ERRFILTER=
endif

## Action for 'make view'
OS=$(shell uname -s)
ifeq ($(OS),Darwin)
PDFVIEWER	?= open
else
PDFVIEWER	?= xdg-open
endif

## Name of the target file, minus .pdf: e.g., TARGET=mypaper causes this
## Makefile to turn mypaper.tex into mypaper.pdf.
TARGET = salicon
TARGETS += $(TARGET)
TEXTARGETS = $(TARGETS:=.tex)
PDFTARGETS = $(TARGETS:=.pdf)
AUXFILES   = $(TARGETS:=.aux)
LOGFILES   = $(TARGETS:=.log)

## If $(TARGET).tex refers to .bib files like \bibliography{foo,bar}, then
## $(BIBFILES) will contain foo.bib and bar.bib, and both files will be added as
## dependencies to $(PDFTARGETS).
## Effect: updating a .bib file will trigger re-typesetting.
BIBFILES = $(patsubst %,%.bib,\
		$(shell grep '^[^%]*\\bibliography{' $(TEXTARGETS) | \
			grep -o '\\bibliography{[^}]\+}' | \
			sed -e 's/^[^%]*\\bibliography{\([^}]*\)}.*/\1/' \
			    -e 's/, */ /g'))

## Add \input'ed or \include'd files to $(PDFTARGETS) dependencies; ignore
## .tex extensions.
INCLUDEDTEX = $(patsubst %,%.tex,\
		$(shell grep '^[^%]*\\\(input\|include\){' $(TEXTARGETS) | \
			grep -o '\\\(input\|include\){[^}]\+}' | \
			sed -e 's/^.*{\([^}]*\)}.*/\1/' \
			    -e 's/\.tex$$//'))

AUXFILES += $(INCLUDEDTEX:.tex=.aux)

## grab a version number from the repository (if any) that stores this.
## * REVISION is the current revision number (short form, for inclusion in text)
## * VCSTURD is a file that gets touched after a repo update
SPACE = $(empty) $(empty)
ifeq ($(shell git status >/dev/null 2>&1 && echo USING_GIT),USING_GIT)
  ifeq ($(shell git svn info >/dev/null 2>&1 && echo USING_GIT_SVN),USING_GIT_SVN)
    # git-svn
    REVISION := $(shell git svn find-rev git-svn)
    VCSTURD := $(subst $(SPACE),\ ,$(shell git rev-parse --git-dir)/refs/remotes/git-svn)
  else
    # plain git
    REVISION := $(shell git describe --always HEAD)
    GIT_BRANCH := $(shell git symbolic-ref HEAD 2>/dev/null)
    VCSTURD := $(subst $(SPACE),\ ,$(shell git rev-parse --git-dir)/$(GIT_BRANCH))
  endif
else ifeq ($(shell hg root >/dev/null 2>&1 && echo USING_HG),USING_HG)
  # mercurial
  REVISION := $(shell hg id -i)
  VCSTURD := $(subst $(SPACE),\ ,$(shell hg root)/.hg/dirstate)
else ifneq ($(wildcard .svn/entries),)
  # subversion
  REVISION := $(subst :,-,$(shell svnversion -n))
  VCSTURD := .svn/entries
endif

# .PHONY names all targets that aren't filenames
.PHONY: all clean pdf view snapshot distill distclean

all: pdf $(AFTERALL)

pdf: $(PDFTARGETS)

view: $(PDFTARGETS)
	$(PDFVIEWER) $(PDFTARGETS)

# define a \Revision{} command you can include in your document's preamble.
# especially useful with e.g. draftfooter.sty or fancyhdr.
# usage: \input{revision}
#        ... \Revision{}
ifneq ($(REVISION),)
REVDEPS += revision.tex
revision.tex: $(VCSTURD)
	/bin/echo '\newcommand{\Revision}'"{$(subst _,\_,$(REVISION))}" > $@
AUXFILES += revision.aux
endif

.INTERMEDIATE: $(AUXFILES)
%.aux: %.tex $(REVDEPS)
	$(PDFLATEX) -draftmode $* $(ERRFILTER)

ifneq ($(strip $(BIBFILES)),)
BIBDEPS = %.bbl
%.bbl: %.aux $(BIBFILES)
	$(BIBTEX) $*
endif

HAS_GLOSSARIES = $(shell \
		grep '^[^%]*\\printglossar\(ies\|y\)' $(TEXTARGETS) $(INCLUDEDTEX) && \
		echo HAS_GLOSSARIES)
ifneq ($(HAS_GLOSSARIES),)
GLSDEPS = %.gls
%.gls: %.aux
	$(MAKEGLOSSARIES) $(TARGETS)
endif

$(PDFTARGETS): %.pdf: %.tex %.aux $(GLSDEPS) $(BIBDEPS) $(INCLUDEDTEX) $(REVDEPS)
	$(PDFLATEX) $* $(ERRFILTER)
ifneq ($(strip $(BIBFILES)),)
	@if egrep -q "undefined (references|citations)" $*.log; then \
		$(BIBTEX) $* && $(PDFLATEX) $* $(ERRFILTER); fi
endif
	@while grep -q "Rerun to" $*.log; do \
		$(PDFLATEX) $* $(ERRFILTER); done

DRAFTS := $(PDFTARGETS:.pdf=-$(REVISION).pdf)
$(DRAFTS): %-$(REVISION).pdf: %.pdf
	cp $< $@
snapshot: $(DRAFTS)

%.distilled.pdf: %.pdf
	gs -q -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$@ \
		-dCompatibilityLevel=1.5 -dPDFSETTINGS=/prepress -c .setpdfwrite -f $<
	exiftool -overwrite_original -Title="" -Creator="" -CreatorTool="" $@

distill: $(PDFTARGETS:.pdf=.distilled.pdf)

distclean: clean
	$(RM) $(PDFTARGETS) $(PDFTARGETS:.pdf=.distilled.pdf) $(EXTRADISTCLEAN)

clean:
	$(RM) $(foreach T,$(TARGETS), \
		$(T).bbl $(T).bcf $(T).bit $(T).blg \
		$(T)-blx.bib $(T).brf $(T).glg $(T).glo \
		$(T).gls $(T).glsdefs $(T).glx \ $(T).gxg \
		$(T).gxs $(T).idx $(T).ilg $(T).ind \
		$(T).ist $(T).loa $(T).lof $(T).lol \
		$(T).lot $(T).maf $(T).mtc $(T).nav \
		$(T).out $(T).pag $(T).run.xml $(T).snm \
		$(T).svn $(T).tdo $(T).tns $(T).toc \
		$(T).vtc $(T).url $(T).synctex.gz $(T).dvi $(T).log $(T).pdf) \
		$(REVDEPS) $(AUXFILES) $(LOGFILES) \
		$(EXTRACLEAN)
